Representing Guardedness in Call-by-Value and Guarded Parametrized Monads

Like the notion of computation via (strong) monads serves to classify various flavours of impurity, including exceptions, non-determinism, probability, local and global store, the notion of guardedness classifies well-behavedness of cycles in various settings. In its most general form, the guardedness discipline applies to general symmetric monoidal categories and further specializes to Cartesian and co-Cartesian categories, where it governs guarded recursion and guarded iteration, respectively. Here, even more specifically, we deal with the semantics of call-by-value guarded iteration. It was shown by Levy, Power and Thielecke that call-by-value languages can be generally interpreted in Freyd categories, but in order to represent effectful function spaces, such a category must canonically arise from a strong monad. We generalize this fact by showing that representing guarded effectful function spaces calls for certain parameterized monads (in the sense of Uustalu). This provides a description of guardedness as an intrinsic categorical property of programs, complementing the existing description of guardedness as a predicate on a category.

==> catprog.tex <==
%
%
%
%
%
%
%
%
%
%

\RequirePackage{bm} 			%
\RequirePackage{mathtools} 		%

\providecommand{\catname}{\mathbf} 
%
\providecommand{\clsname}{\mathcal}
\providecommand{\oname}[1]{\operatorname{\mathsf{#1}}}

%
\def\defcatname#1{\expandafter\def\csname B#1\endcsname{\catname{#1}}}
\def\defcatnames#1{\ifx#1\defcatnames\else\defcatname#1\expandafter\defcatnames\fi}
\defcatnames ABCDEFGHIJKLMNOPQRSTUVWXYZ\defcatnames

%
\def\defclsname#1{\expandafter\def\csname C#1\endcsname{\clsname{#1}}}
\def\defclsnames#1{\ifx#1\defclsnames\else\defclsname#1\expandafter\defclsnames\fi}
\defclsnames ABCDEFGHIJKLMNOPQRSTUVWXYZ\defclsnames

%
\def\defbbname#1{\expandafter\def\csname BB#1\endcsname{{\bm{\mathsf{#1}}}}}
\def\defbbnames#1{\ifx#1\defbbnames\else\defbbname#1\expandafter\defbbnames\fi}
\defbbnames ABCDEFGHIJKLMNOPQRSTUVWXYZ\defbbnames

%
\def\defbbname#1{\expandafter\def\csname BM#1\endcsname{{\bm{\mathsf{#1}}}}}
\def\defbbnames#1{\ifx#1\defbbnames\else\defbbname#1\expandafter\defbbnames\fi}
\defbbnames ABCDEFGHIJKLMNOPQRSTUVWXYZ\defbbnames

%
\def\Set{\catname{Set}}
\def\Cpo{\catname{Cpo}}
\def\Cppo{\catname{Cppo}}
\def\dCpo{\catname{dCpo}}
\def\DCpo{\catname{DCpo}}
\def\Top{\catname{Top}}
\def\Met{\catname{Met}}
\def\Rel{\catname{Rel}}

%
\providecommand{\eps}{{\operatorname\epsilon}}
\providecommand{\ups}{{\operatorname\upsilon}}
\providecommand{\amp}{\mathbin{\&}}

\providecommand{\argument}{\operatorname{-\!-}}
\providecommand{\altargument}{\underline{\;\;}}

\providecommand{\wave}[1]{\widetilde{#1}}			%
\providecommand{\ul}{\underline}				%

\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\providecommand{\mplus}{{\scriptscriptstyle\bf+}} 	 	%

\providecommand{\smin}{\smallsetminus}

\providecommand{\ass}{\mathrel{\coloneqq}}
\providecommand{\bnf}{\mathrel{\Coloneqq}}

%
\providecommand{\PSet}{{\mathcal P}}				%
\providecommand{\FSet}{{\mathcal P}_{\omega}}			%
\providecommand{\CSet}{{\mathcal P}_{\omega_1}}			%
\providecommand{\NESet}{{\mathcal P}^{\mplus}}			%
\providecommand{\Id}{\operatorname{Id}}

%
\providecommand{\Hom}{\mathsf{Hom}}
\providecommand{\id}{\mathsf{id}}
\providecommand{\op}{\mathsf{op}}
\providecommand{\comp}{\mathbin{\circ}}
\providecommand{\iso}{\mathbin{\cong}}
\providecommand{\tensor}{\mathbin{\otimes}}
\providecommand{\unit}{\star}
\providecommand{\bang}{\operatorname!}				%

%
\providecommand{\from}{\leftarrow}

\providecommand{\ito}{\hookrightarrow}				%
\providecommand{\sto}{\twoheadrightarrow}			%

\providecommand{\ifrom}{\hookleftarrow}				

\providecommand{\pto}{\mathrel{\rightharpoonup}}		%
\providecommand{\pfrom}{\mathrel{\leftarpoonup}}		%

\providecommand{\tto}{\mathrel{\Rightarrow}}			%
\providecommand{\tfrom}{\mathrel{\Leftarrow}}			%

\providecommand{\mto}{\mapsto}

\providecommand{\xto}[1]{\,\xrightarrow{#1}\,}
\providecommand{\xfrom}[1]{\,\xleftarrow{\;#1}\,}

\providecommand{\To}{\mathrel{\Rightarrow}}			%
\providecommand{\From}{\mathrel{\Leftarrow}}			

\providecommand{\dar}{\kern-.75pt\operatorname{\downarrow}}
\providecommand{\uar}{\kern-.75pt\operatorname{\uparrow}}

\providecommand{\Dar}{\kern-.75pt\operatorname{\Downarrow}}
\providecommand{\Uar}{\kern-.75pt\operatorname{\Uparrow}}


%
\providecommand{\True}{\top}
\providecommand{\False}{\bot}

\providecommand{\bigor}{\bigvee}
\providecommand{\bigand}{\bigwedge}

\providecommand{\impl}{\Rightarrow}
\providecommand{\equ}{\Longleftrightarrow}

\providecommand{\entails}{\vdash}

%
\providecommand{\appr}{\sqsubseteq}
\providecommand{\join}{\sqcup}
\providecommand{\meet}{\sqcap}

\providecommand{\bigjoin}{\bigsqcup}
\providecommand{\bigmeet}{\bigsqcap}

%
\providecommand{\fst}{\oname{fst}}
\providecommand{\snd}{\oname{snd}}
\providecommand{\pr}{\oname{pr}}

\providecommand{\brks}[1]{\langle #1\rangle}
\providecommand{\Brks}[1]{\bigl\langle #1\bigr\rangle}

%
\providecommand{\inl}{\oname{inl}}
\providecommand{\inr}{\oname{inr}}
\providecommand{\inj}{\oname{in}}

\DeclareSymbolFont{Symbols}{OMS}{cmsy}{m}{n}
\DeclareMathSymbol{\iobj}{\mathord}{Symbols}{"3B}
%

%
\providecommand{\curry}{\oname{curry}}
\providecommand{\uncurry}{\oname{uncurry}}
\providecommand{\ev}{\oname{ev}}

%
\RequirePackage{stmaryrd}

\providecommand{\lsem}{\llbracket}
\providecommand{\rsem}{\rrbracket}
\providecommand{\sem}[1]{\lsem #1 \rsem}

\providecommand{\Lsem}{\bigl\llbracket}
\providecommand{\Rsem}{\bigr\rrbracket}
\providecommand{\Sem}[1]{\Lsem #1 \Rsem}

%
\providecommand{\comma}{,\operatorname{}\linebreak[1]}	 %
\providecommand{\dash}{\nobreakdash-\hspace{0pt}}	 %
\providecommand{\erule}{\rule{0pt}{0pt}}		 %
                                                         %

\providecommand{\by}[1]{\text{/\!\!/~#1}}		 %
\providecommand{\pacman}[1]{}				 %

\newcommand{\undefine}[1]{\let #1\relax}		 %

\providecommand{\noqed}{\def\qed{}}			 %

%
\providecommand{\mone}{{\text{\kern.5pt\rmfamily-}\mathsf{\kern-.5pt1}}}

\makeatletter
\@ifpackageloaded{enumitem}{}{
  \RequirePackage[loadonly]{enumitem}			 %
}                                                        %
\makeatother

%
\newlist{citemize}{itemize}{1}
\setlist[citemize]{label=\labelitemi,wide} 
%

\newlist{cenumerate}{enumerate}{1}
\setlist[cenumerate,1]{label=\arabic*.~,ref={\arabic*},wide} 
%

%
%
 
%
\makeatletter
\def\mfix#1{\oname{#1}\@ifnextchar\bgroup\@mfix{}}	 %
\def\@mfix#1{#1\@ifnextchar\bgroup\mfix{}}		 %
\makeatother

%
\providecommand{\ift}[3]{\mfix{if}{\mathbin{}#1}{then}{\mathbin{}#2}{else}{\mathbin{}#3}}
\providecommand{\case}[3]{\mfix{case}{\mathbin{}#1}{of}{#2}{\kern-1pt;}{\mathbin{}#3}}



